Watch Before You Answer: Learning from Visually Grounded Post-Training

It is critical for vision-language models (VLMs) to comprehensively understand visual, temporal, and textual cues. However, despite rapid progress in multimodal modeling, video understanding performance still lags behind text-based reasoning. In this work, we find that progress is even worse than previously assumed: commonly reported long video understanding benchmarks contain 40-60% of questions that can be answered using text cues alone. Furthermore, we find that these issues are also pervasive in widely used post-training datasets, potentially undercutting the ability of post-training to improve VLM video understanding performance. Guided by this observation, we introduce VidGround as a simple yet effective solution: using only the actual visually grounded questions without any linguistic biases for post-training. When used in tandem with RL-based post-training algorithms, this simple technique improves performance by up to 6.2 points relative to using the full dataset, while using only 69.1% of the original post-training data. Moreover, we show that data curation with a simple post-training algorithm outperforms several more complex post-training techniques, highlighting that data quality is a major bottleneck for improving video understanding in VLMs. These results underscore the importance of curating post-training data and evaluation benchmarks that truly require visual grounding to advance the development of more capable VLMs. Project page: http://vidground.etuagi.com.

==> tables/frame_scaling.tex <==

\begin{table*}[H]
\centering
\caption{Performance of VLMs with frame scaling across LVU benchmarks.}
\label{tab:video_model_performance}

\begingroup
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
Models & Frames & VideoMME & VideoMMMU (P) & VideoMMMU (C) & MMVU \\
\midrule
\multirow{3}{*}{Qwen2.5-VL-7B} & 16 & 58.11 & 62.67 & 48.33 & 45.50 \\
 & 32 & 60.67 & 62.33 & 49.00 & 47.10 \\
 & 64 & 62.30 & 63.00 & 47.67 & 47.00 \\
\midrule
\multirow{3}{*}{MiMo-VL-7B-RL} & 16 & 58.00 & 69.00 & 41.00 & 48.70 \\
 & 32 & 61.96 & 71.67 & 41.67 & 48.90  \\
 & 64 & 64.81 & 72.67 & 41.33 & 49.20  \\
\midrule
\multirow{3}{*}{LLaVA-Critic-R1-7B} & 16 & 57.59 & 63.67 & 47.33 & 47.80  \\
 & 32 & 60.74 & 65.33 & 54.00 & 47.30  \\
 & 64 & 61.78 & 59.33 & 47.67 & 47.40  \\
\midrule
\multirow{3}{*}{LLaVA-Critic-R1-7B-Plus-Qwen} & 16 & 58.11 & 64.67 & 46.33 & 46.70 \\
 & 32 & 61.41 & 65.00 & 49.00 & 47.50 \\
 & 64 & 62.48 & 61.00 & 48.67 & 49.10 \\
\bottomrule
\end{tabular}
}%
\endgroup
\end{table*}

==> tables/train_other_rl.tex <==
\begin{table*}[htbp]
\centering
\caption{Full performance comparison of RL-based post-training methods on video understanding benchmarks (VideoMME~\cite{fu2025video}, VideoMMMU~\cite{hu2025video}, MMVU~\cite{zhao2025mmvu}). All methods use Qwen2.5-VL-7B~\cite{bai2025qwen2} as the base model. Models are evaluated at 16, 32, and 64 frames per video. Full = all benchmark questions; VG = visually grounded question subset (questions that require video to answer). Avg.\ columns report mean accuracy across three benchmarks, with deltas showing improvement over the Qwen2.5-VL-7B base model: {\small\color{teal}($+x$)} and {\small\color{red!80!black}($-x$)}. Bold indicates best; \colorbox{secondcolor}{highlighted} rows are ours.}
\label{tab:train_other_rl}
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{cl|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Frames}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{VideoMME}} & \multicolumn{2}{c|}{\textbf{VideoMMMU}} & \multicolumn{2}{c|}{\textbf{MMVU}} & \multicolumn{2}{c}{\textbf{Avg.}} \\
 & & Full & VG & Full & VG & Full & VG & Full & VG \\ \midrule
\multirow{7}{*}{16} & Qwen2.5-VL-7B  & 58.2 & 47.7 & 45.0 & 35.2 & 60.5 & 45.9 & 54.6\phantom{{\small (+0.0)}} & 42.9\phantom{{\small (+0.0)}} \\
 & TW-GRPO & 58.2 & 47.6 & \textbf{48.6} & 37.2 & 61.8 & 47.6 & 56.2 {\small\color{teal}($+$1.6)} & 44.1 {\small\color{teal}($+$1.2)} \\
 & LongVILA-R1-7B  & 55.5 & 44.6 & 38.8 & 29.5 & 59.1 & 44.9 & 51.1 {\small\color{red!80!black}($-$3.5)} & 39.7 {\small\color{red!80!black}($-$3.2)} \\
 & Video-RTS & \textbf{58.7} & 47.4 & 47.1 & 37.6 & 61.8 & 45.6 & 55.9 {\small\color{teal}($+$1.3)} & 43.5 {\small\color{teal}($+$0.6)} \\
 & Qwen2.5-VL-7B-SFT  & 58.2 & 46.2 & 43.1 & 35.1 & 51.3 & 42.1 & 50.9 {\small\color{red!80!black}($-$3.7)} & 41.1 {\small\color{red!80!black}($-$1.8)} \\
 & Video-R1  & 56.9 & 45.3 & 44.7 & 35.4 & 54.5 & 44.5 & 52.0 {\small\color{red!80!black}($-$2.6)} & 41.7 {\small\color{red!80!black}($-$1.2)} \\
 & \textbf{\ours{}}  & \cellcolor{secondcolor}\textbf{58.7} & \cellcolor{secondcolor}\textbf{48.5} & \cellcolor{secondcolor}47.4 & \cellcolor{secondcolor}\textbf{38.2} & \cellcolor{secondcolor}\textbf{64.2} & \cellcolor{secondcolor}\textbf{49.0} & \cellcolor{secondcolor}\textbf{56.8} {\small\textbf{\color{teal}($+$2.2)}} & \cellcolor{secondcolor}\textbf{45.2} {\small\textbf{\color{teal}($+$2.3)}} \\ \midrule
\multirow{7}{*}{32} & Qwen2.5-VL-7B  & 60.7 & 50.8 & 45.4 & 34.5 & 62.3 & 48.0 & 56.1\phantom{{\small (+0.0)}} & 44.4\phantom{{\small (+0.0)}} \\
 & TW-GRPO  & 61.2 & 51.6 & 47.9 & 38.9 & 63.1 & 47.3 & 57.4 {\small\color{teal}($+$1.3)} & 45.9 {\small\color{teal}($+$1.5)} \\
 & LongVILA-R1-7B  & 60.2 & 50.9 & 40.7 & 31.0 & 61.5 & 46.9 & 54.1 {\small\color{red!80!black}($-$2.0)} & 42.9 {\small\color{red!80!black}($-$1.5)} \\
 & Video-RTS & 61.3 & 51.2 & 47.7 & 37.0 & 65.0 & 50.7 & 58.0 {\small\color{teal}($+$1.9)} & 46.3 {\small\color{teal}($+$1.9)} \\
 & Qwen2.5-VL-7B-SFT  & 60.7 & 50.7 & 47.8 & \textbf{40.0} & 51.0 & 43.2 & 53.2 {\small\color{red!80!black}($-$2.9)} & 44.6 {\small\color{teal}($+$0.2)} \\
 & Video-R1  & 60.2 & 49.5 & 45.4 & 36.0 & 56.2 & 43.8 & 53.9 {\small\color{red!80!black}($-$2.2)} & 43.1 {\small\color{red!80!black}($-$1.3)} \\
 & \textbf{\ours{}}  & \cellcolor{secondcolor}\textbf{61.5} & \cellcolor{secondcolor}\textbf{51.8} & \cellcolor{secondcolor}\textbf{48.3} & \cellcolor{secondcolor}39.5 & \cellcolor{secondcolor}\textbf{65.8} & \cellcolor{secondcolor}\textbf{51.4} & \cellcolor{secondcolor}\textbf{58.5} {\small\textbf{\color{teal}($+$2.4)}} & \cellcolor{secondcolor}\textbf{47.6} {\small\textbf{\color{teal}($+$3.2)}} \\ \midrule
\multirow{7}{*}{64} & Qwen2.5-VL-7B  & 62.3 & 52.6 & 46.6 & 38.2 & 62.6 & 48.0 & 57.2\phantom{{\small (+0.0)}} & 46.3\phantom{{\small (+0.0)}} \\
 & TW-GRPO  & 62.7 & \textbf{53.7} & 48.3 & \textbf{40.6} & 64.2 & \textbf{50.3} & 58.4 {\small\color{teal}($+$1.2)} & \textbf{48.2} {\small\color{teal}($+$1.9)} \\
 & LongVILA-R1-7B & 61.6 & 51.2 & 41.2 & 31.1 & 58.8 & 43.8 & 53.9 {\small\color{red!80!black}($-$3.3)} & 42.0 {\small\color{red!80!black}($-$4.3)} \\
 & Video-RTS & 62.9 & 53.3 & 46.4 & 36.6 & 63.9 & 49.3 & 57.7 {\small\color{teal}($+$0.5)} & 46.4 {\small\color{teal}($+$0.1)} \\
 & Qwen2.5-VL-7B-SFT  & 62.2 & 51.7 & 47.6 & 40.1 & 55.4 & 45.6 & 55.1 {\small\color{red!80!black}($-$2.1)} & 45.8 {\small\color{red!80!black}($-$0.5)} \\
 & Video-R1  & 61.2 & 50.3 & 45.4 & 37.2 & 53.2 & 41.1 & 53.3 {\small\color{red!80!black}($-$3.9)} & 42.9 {\small\color{red!80!black}($-$3.4)} \\
 & \textbf{\ours{}}  & \cellcolor{secondcolor}\textbf{63.4} & \cellcolor{secondcolor}\textbf{53.7} & \cellcolor{secondcolor}\textbf{49.4} & \cellcolor{secondcolor}39.9 & \cellcolor{secondcolor}\textbf{65.6} & \cellcolor{secondcolor}50.0 & \cellcolor{secondcolor}\textbf{59.5} {\small\textbf{\color{teal}($+$2.3)}} & \cellcolor{secondcolor}47.9 {\small\color{teal}($+$1.6)} \\ \bottomrule
\end{tabular}
}
\end{table*}


